Chemical bonding, elasticity, and valence force field models: a case study for alpha-Pt_2Si and PtSi

We have carried out a detailed study of the chemical bonding for two room-temperature stable platinum silicide phases, tetragonal alpha-Pt_2Si and orthorhombic PtSi. An analysis of the valence electronic charge density reveals surprising evidence of covalent three-center bonds in both silicide phases, as well as two-dimensional metallic sheets in alpha-Pt_2Si. These elements of the bonding are further analyzed by constructing valence force field models using the results from recent first principles calculations of the six (nine) independent, non-zero elastic constants of alpha-Pt_2Si (PtSi). The resulting volume-, radial-, and angular-dependent force constants provide insight into the relative strength of various bonding elements as well as the trends observed in the elastic constants themselves. The valence force field analysis yields quantitative information about the nature of the chemical bonding which is not easily discernable from the more qualitative charge density plots. More generally, this study demonstrates that the detailed variations in the elastic constants of a material contain useful information about the chemical bonds which can be extracted using valence force field models. Inversely, these models also allow identification of specific elements of the chemical bonding with particular trends in the elastic constants, both within a given material and among a class of related materials.

==> prmulticol.tex <==
% Phys-Rev-TeX-files twocolumn

% \narrowtext and \widetext are redefined using the multicol package
% such that we can switch back and forth between narrow and wide
% text. Note that we have to terminate every \narrowtext with \widetext

% Works fine with revtex-3.1

% Roland Winkler

\RequirePackage{multicol}

\newif\ifmynarrow \mynarrowfalse

\parskip 0pt %plus 1pt

\renewcommand{\narrowtext}{%
  \ifmynarrow\hspace*{\fill}\raisebox{-1ex}[0pt][0pt]{%
    \rule{0.3pt}{1ex}%
    \rule[1ex]{20.5pc}{0.3pt}}\fi
  \mynarrowtrue
  \vspace{-1.0ex}%
  \begin{multicols}{2}%
  \par\global\columnwidth20.5pc
  \global\hsize\columnwidth\global\linewidth\columnwidth
  \global\displaywidth\columnwidth}

\renewcommand{\widetext}{%
  \end{multicols}%
  \vspace{-2.5ex}%
  \noindent\raisebox{1ex}[0pt][0pt]{%
    \rule{20.5pc}{0.3pt}%
    \rule{0.3pt}{1ex}}%
  \par\global\columnwidth42.5pc
  \global\hsize\columnwidth\global\linewidth\columnwidth
  \global\displaywidth\columnwidth}

